DANSK and DaCy 2.6.0: Domain Generalization of Danish Named Entity Recognition

Named entity recognition is one of the cornerstones of Danish NLP, essential for language technology applications within both industry and research. However, Danish NER is inhibited by a lack of available datasets. As a consequence, no current models are capable of fine-grained named entity recognition, nor have they been evaluated for potential generalizability issues across datasets and domains. To alleviate these limitations, this paper introduces: 1) DANSK: a named entity dataset providing for high-granularity tagging as well as within-domain evaluation of models across a diverse set of domains; 2) DaCy 2.6.0 that includes three generalizable models with fine-grained annotation; and 3) an evaluation of current state-of-the-art models' ability to generalize across domains. The evaluation of existing and new models revealed notable performance discrepancies across domains, which should be addressed within the field. Shortcomings of the annotation quality of the dataset and its impact on model training and evaluation are also discussed. Despite these limitations, we advocate for the use of the new dataset DANSK alongside further work on the generalizability within Danish NER.

==> tabs/automated_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|p{1.5cm}|p{5cm}|p{5cm}|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Initial annotation}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Streamlined annotation}} \\ \hline
Rater 1 & \thead{{[}Mette F.{]} (PER) er \\statsminister i {[}DK{]} (GPE)} & \thead{{[}Mette F.{]} (PER) er \\statsminister i {[}DK{]} (GPE)} \\ \hline
\rowcolor[HTML]{EFEFEF}
Rater 3 & \thead{{[}Mette F.{]} (PER) er \\statsminister i {[}DK{]} (GPE)} & \thead{{[}Mette F.{]} (PER) er \\statsminister i {[}DK{]} (GPE)} \\ \hline
Rater 5 & \thead{{[}Mette{]} (PER) F. er \\statsminister i DK}             & \thead{{[}Mette{]} (PER) F. er \\statsminister i {[}DK{]} (GPE)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
Rater 9 & \thead{{[}Mette{]} (PER) F. er \\{[}statsminister{]} (PER) i DK} & \thead{{[}Mette{]} (PER) F. er \\statsminister i {[}DK{]} (GPE)} \\ \hline
\end{tabular}


==> tabs/full_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
             & \textbf{Sum} & \textbf{Conversation} & \textbf{Dannet} & \textbf{Legal} & \textbf{News} & \textbf{Social Media} & \textbf{Web} & \textbf{Wiki} \\ \hline
Texts         & 15062        & 1649                  & 25              & 2163           & 421           & 554                   & 8270         & 1709                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
Named entities         & 14462        & 1286                  & 23              & 1637           & 496           & 329                   & 9309         & 1156                   \\ \hline
CARDINAL     & 2096         & 419                   & 10              & 128            & 43            & 27                    & 1392         & 77                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
DATE         & 1756         & 142                   & 6               & 323            & 50            & 38                    & 1017         & 168                    \\ \hline
EVENT        & 211          & 52                    & 0               & 1              & 10            & 3                     & 127          & 13                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
FACILITY     & 246          & 3                     & 1               & 4              & 18            & 3                     & 198          & 15                     \\ \hline
GPE          & 1604         & 166                   & 3               & 73             & 85            & 34                    & 1063         & 167                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
LANGUAGE     & 126          & 3                     & 0               & 0              & 0             & 0                     & 97           & 26                     \\ \hline
LAW          & 183          & 15                    & 0               & 119            & 1             & 0                     & 33           & 13                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
LOCATION     & 424          & 20                    & 0               & 2              & 8             & 8                     & 346          & 38                     \\ \hline
MONEY        & 714          & 3                     & 0               & 85             & 15            & 24                    & 587          & 0                      \\ \hline
\rowcolor[HTML]{EFEFEF} 
NORP         & 495          & 83                    & 0               & 72             & 26            & 4                     & 229          & 59                     \\ \hline
ORDINAL      & 127          & 14                    & 0               & 22             & 9             & 3                     & 49           & 29                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
ORGANIZATION & 2507         & 104                   & 0               & 521            & 71            & 48                    & 1680         & 71                     \\ \hline
PERCENT      & 148          & 5                     & 0               & 13             & 12            & 0                     & 112          & 4                      \\ \hline
\rowcolor[HTML]{EFEFEF} 
PERSON       & 2133         & 224                   & 3               & 239            & 120           & 81                    & 1164         & 158                    \\ \hline
PRODUCT      & 763          & 3                     & 0               & 10             & 2             & 36                    & 705          & 5                      \\ \hline
\rowcolor[HTML]{EFEFEF} 
QUANTITY     & 292          & 1                     & 0               & 11             & 8             & 19                    & 220          & 32                     \\ \hline
TIME         & 218          & 16                    & 0               & 5              & 15            & 1                     & 175          & 6                      \\ \hline
\rowcolor[HTML]{EFEFEF} 
WORK OF ART  & 419          & 13                    & 0               & 9              & 3             & 0                     & 115          & 275                    \\ \hline
\end{tabular}
\end{scriptsize}

% \begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
%              & \thead{\textbf{Sum}} & \thead{\textbf{Conversation}} & \thead{\textbf{Dannet}} & \thead{\textbf{Legal}} & \thead{\textbf{News}} & \thead{\textbf{Social}\\ \textbf{Media}} & \thead{\textbf{Web}} & \thead{\textbf{Wiki}\\ \textbf{and}\\ \textbf{Books}} \\ \hline
% DOCS         & 15062                         & 1649                  & 25              & 2163           & 421           & 554                   & 8270         & 1709                    \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% ENTS         & 14462                         & 1286                  & 23              & 1637           & 496           & 329                   & 9309         & 1156                    \\ \hline
% CARDINAL     & 2096                          & 419                   & 10              & 128            & 43            & 27                    & 1392         & 77                      \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% DATE         & 1756                          & 142                   & 6               & 323            & 50            & 38                    & 1017         & 168                     \\ \hline
% EVENT        & 211                           & 52                    & 0               & 1              & 10            & 3                     & 127          & 13                      \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% FACILITY     & 246                           & 3                     & 1               & 4              & 18            & 3                     & 198          & 15                      \\ \hline
% GPE          & 1604                          & 166                   & 3               & 73             & 85            & 34                    & 1063         & 167                     \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% LANGUAGE     & 126                           & 3                     & 0               & 0              & 0             & 0                     & 97           & 26                      \\ \hline
% LAW          & 183                           & 15                    & 0               & 119            & 1             & 0                     & 33           & 13                      \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% LOCATION     & 424                           & 20                    & 0               & 2              & 8             & 8                     & 346          & 38                      \\ \hline
% MONEY        & 714                           & 3                     & 0               & 85             & 15            & 24                    & 587          & 0                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% NORP         & 495                           & 83                    & 0               & 72             & 26            & 4                     & 229          & 59                      \\ \hline
% ORDINAL      & 127                           & 14                    & 0               & 22             & 9             & 3                     & 49           & 29                      \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% ORGANIZATION & 2507                          & 104                   & 0               & 521            & 71            & 48                    & 1680         & 71                      \\ \hline
% PERCENT      & 148                           & 5                     & 0               & 13             & 12            & 0                     & 112          & 4                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% PERSON       & 2133                          & 224                   & 3               & 239            & 120           & 81                    & 1164         & 158                     \\ \hline
% PRODUCT      & 763                           & 3                     & 0               & 10             & 2             & 36                    & 705          & 5                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% QUANTITY     & 292                           & 1                     & 0               & 11             & 8             & 19                    & 220          & 32                      \\ \hline
% TIME         & 218                           & 16                    & 0               & 5              & 15            & 1                     & 175          & 6                       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% WORK OF ART  & 419                           & 13                    & 0               & 9              & 3             & 0                     & 115          & 275                     \\ \hline
% \end{tabular}


==> tabs/full_tags.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
               & \textbf{Full}  & \textbf{Train}           & \textbf{Validation} & \textbf{Test}           \\ \hline
Texts           & 15062 & 12062 (80\%)    & 1500 (10\%)         & 1500 (10\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
Named entities & 14462 & 11638 (80.5\%) & 1327 (9.2\%)       & 1497 (10.3\%) \\ \hline
CARDINAL       & 2069  & 1702 (82.3\%)  & 168 (8.1\%)        & 226 (11\%)  \\ \hline
\rowcolor[HTML]{EFEFEF} 
DATE           & 1756  & 1411 (80.4\%)  & 182 (10.4\%)       & 163 (9.3\%)   \\ \hline
EVENT          & 211   & 175 (82.9\%)   & 19 (9\%)         & 17 (8.1\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
FACILITY       & 246   & 200 (81.3\%)   & 25 (10.2\%)        & 21 (8.5\%)    \\ \hline
GPE            & 1604  & 1276 (79.6\%)  & 135 (8.4\%)        & 193 (12\%)  \\ \hline
\rowcolor[HTML]{EFEFEF} 
LANGUAGE       & 126   & 147 (59.5\%)    & 44 (17.8\%)        & 56 (22.7\%)   \\ \hline
LAW            & 183   & 148 (80.9\%)   & 17 (9.3\%)         & 18 (9.8\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
LOCATION       & 424   & 351 (82.8\%)   & 46 (10.9\%)        & 27 (6.4\%)    \\ \hline
MONEY          & 714   & 566 (79.3\%)   & 72 (10.1\%)        & 76 (10.6\%)   \\ \hline
\rowcolor[HTML]{EFEFEF} 
NORP           & 495   & 405 (81.8\%)   & 41 (8.3\%)         & 49 (9.9\%)    \\ \hline
ORDINAL        & 127   & 105 (82.7\%)   & 11 (8.7\%)         & 11 (8.7\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
ORGANIZATION   & 2507  & 1960 (78.2\%)  & 249 (9.9\%)        & 298 (11.9\%)  \\ \hline
PERCENT        & 148   & 123 (83.1\%)   & 13 (8.8\%)         & 12 (8.1\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
PERSON         & 2133  & 1767 (82.8\%)  & 191 (8\%)        & 175 (8.2\%)   \\ \hline
PRODUCT        & 763   & 634 (83.1\%)   & 57 (7.5\%)         & 72 (9.4\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
QUANTITY       & 292   & 242 (82.9\%)   & 28 (9.6\%)         & 22 (7.5\%)    \\ \hline
TIME           & 218   & 185 (84.9\%)   & 18 (8.3\%)         & 15 (6.9\%)    \\ \hline
\rowcolor[HTML]{EFEFEF} 
WORK OF ART    & 419   & 335 (79\%)   & 38 (9.1\%)         & 46 (10\%)   \\ \hline
\end{tabular}


==> tabs/general_sources.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Domain} & \textbf{Source}    & \textbf{Full} & \textbf{Train} & \textbf{Dev} & \textbf{Test} \\ \hline
\rowcolor[HTML]{FFFFFF} 
Conversation    & Europa Parlamentet & 206           & 173            & 17           & 16            \\ \hline
\rowcolor[HTML]{EFEFEF} 
Conversation    & Folketinget        & 23            & 21             & 1            & 1             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Conversation    & NAAT               & 554           & 431            & 50           & 73            \\ \hline
\rowcolor[HTML]{EFEFEF} 
Conversation    & OpenSubtitles      & 377           & 300            & 39           & 38            \\ \hline
\rowcolor[HTML]{FFFFFF} 
Conversation    & Spontaneous speech & 489           & 395            & 54           & 40            \\ \hline
\rowcolor[HTML]{EFEFEF} 
Dannet          & Dannet             & 25            & 18             & 4            & 3             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Legal           & Retsinformation.dk & 965           & 747            & 105          & 113           \\ \hline
\rowcolor[HTML]{EFEFEF} 
Legal           & Skat.dk            & 471           & 364            & 53           & 54            \\ \hline
\rowcolor[HTML]{FFFFFF} 
Legal           & Retspraktis        & 727           & 579            & 76           & 72            \\ \hline
\rowcolor[HTML]{EFEFEF} 
News            & DanAvis            & 283           & 236            & 20           & 27            \\ \hline
\rowcolor[HTML]{FFFFFF} 
News            & TV2R               & 138           & 110            & 16           & 12            \\ \hline
\rowcolor[HTML]{EFEFEF} 
Social Media    & hestenettet.dk     & 554           & 439            & 51           & 64            \\ \hline
\rowcolor[HTML]{FFFFFF} 
Web             & Common Crawl       & 8270          & 6661           & 826          & 783           \\ \hline
\rowcolor[HTML]{EFEFEF} 
Wiki \& Books   & adl                & 640           & 517            & 57           & 66            \\ \hline
\rowcolor[HTML]{FFFFFF} 
Wiki \& Books   & Wikipedia          & 279           & 208            & 30           & 41            \\ \hline
\rowcolor[HTML]{EFEFEF} 
Wiki \& Books   & WikiBooks          & 335           & 265            & 36           & 34            \\ \hline
\rowcolor[HTML]{FFFFFF} 
Wiki \& Books   & WikiSource         & 455           & 371            & 43           & 41            \\ \hline
\end{tabular}


==> tabs/initial_kappa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{tabular}{ll}
% \toprule
% \multicolumn{2}{c}{\textbf{Average Cohen's $\kappa$}} \\ 
% \midrule
% \midrule
% Annotator 1  & 0.6                            \\       
   
% Annotator 2  & 0.52                           \\       
% Annotator 3  & 0.51                           \\       
   
% Annotator 4  & 0.58                           \\       
% Annotator 5  & 0.54                           \\       
   
% Annotator 6  & 0.56                           \\       
% Annotator 7  & 0.47                           \\       
   
% Annotator 8  & 0.51                           \\       
% Annotator 9  & 0.52                           \\       
   
% Annotator 10 & 0.56                           \\       
% \end{tabular}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{tabular}{ll}
% \toprule
% \multicolumn{2}{c}{\textbf{Average Cohen's $\kappa$ (Initial)}} \\ 
% \midrule
% \midrule
% Annotator 1  & 0.6                            \\   
   
% Annotator 2  & 0.52                           \\   
% Annotator 3  & 0.51                           \\   
   
% Annotator 4  & 0.58                           \\   
% Annotator 5  & 0.54                           \\   
   
% Annotator 6  & 0.56                           \\   
% Annotator 7  & 0.47                           \\   
   
% Annotator 8  & 0.51                           \\   
% Annotator 9  & 0.52                           \\   
   
% Annotator 10 & 0.56                           \\   
% \end{tabular}


\begin{tabular}{ll}
\toprule
\multicolumn{2}{c}{\textbf{Average Cohen's $\kappa$ (Initial)}} \\ 
\midrule
\midrule   
Annotator 1  & 0.6                            \\       
\rowcolor[HTML]{EFEFEF} 
Annotator 2  & 0.52                           \\       
Annotator 3  & 0.51                           \\       
\rowcolor[HTML]{EFEFEF} 
Annotator 4  & 0.58                           \\       
Annotator 5  & 0.54                           \\       
\rowcolor[HTML]{EFEFEF} 
Annotator 6  & 0.56                           \\       
Annotator 7  & 0.47                           \\       
\rowcolor[HTML]{EFEFEF} 
Annotator 8  & 0.51                           \\       
Annotator 9  & 0.52                           \\       
\rowcolor[HTML]{EFEFEF} 
Annotator 10 & 0.56                           \\       
\end{tabular}


==> tabs/sota_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\centering
\begin{tabular}{|c|ccc|c|ccc|ccc|}
\hline
\rowcolor[HTML]{EFEFEF} 
               & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DaCy fine-grained}}                                                                  & \textbf{ScandiNER}       & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DaCy}}                                                                               & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{spaCy}}                                                                     \\ \hline
               & \multicolumn{1}{c|}{\textbf{Large}}                        & \multicolumn{1}{c|}{\textbf{Medium}}                       & \textbf{Small} & \textbf{Base-ner-scandi} & \multicolumn{1}{c|}{\textbf{Large}}                        & \multicolumn{1}{c|}{\textbf{Medium}}                       & \textbf{Small} & \multicolumn{1}{c|}{\textbf{Large}}               & \multicolumn{1}{c|}{\textbf{Medium}}                       & \textbf{Small} \\ \hline
\rowcolor[HTML]{EFEFEF} 
Across domains & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.87}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.85}} & 0.80           & 0.64                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.68}          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.63}          & 0.51           & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.49} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.49}          & 0.31           \\ \hline
Conversation   & \multicolumn{1}{c|}{0.81}                                  & \multicolumn{1}{c|}{\textbf{0.85}}                         & \textit{0.82}  & 0.66                     & \multicolumn{1}{c|}{0.74}                                  & \multicolumn{1}{c|}{0.71}                                  & 0.68           & \multicolumn{1}{c|}{0.72}                         & \multicolumn{1}{c|}{\textit{0.73}}                         & 0.69           \\ \hline
\rowcolor[HTML]{EFEFEF} 
Legal          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.90}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.91}} & 0.88           & 0.59                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.70}          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.76}          & 0.612          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.56} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.58}          & 0.44           \\ \hline
\rowcolor[HTML]{FFFFFF} 
News           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.9}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.8}           & 0.8            & 0.67                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textit{0.85}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.68}          & 0.66           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.61} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.61}          & 0.64           \\ \hline
\rowcolor[HTML]{EFEFEF} 
Social Media   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.74}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.74}} & 0.56           & 0.71                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.74}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.78}} & 0.35           & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.63} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.74}} & 0.46           \\ \hline
\rowcolor[HTML]{FFFFFF} 
Web            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.88}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textit{0.84}} & 0.78           & \textit{0.63}            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.65}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.58}          & 0.46           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.44} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.45}          & 0.25           \\ \hline
\rowcolor[HTML]{EFEFEF} 
Wiki and Books & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.82}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.89}} & 0.76           & 0.80                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{0.73}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.72}          & 0.62           & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.52} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.50}          & 0.32           \\ \hline
\end{tabular}

==> tabs/sota_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Framework} & \textbf{Model}  & \textbf{F1}                  & \textbf{Recall}              & \textbf{Precision}           \\ \hline
\rowcolor[HTML]{EFEFEF} 
NbAI-lab           & Base-ner-scandi & \textit{0.64}                & 0.59                         & \textbf{0.698}               \\ \hline
\rowcolor[HTML]{FFFFFF} 
DaCy               & Large           & \textbf{0.68}                & 0.673                        & \textit{0.688}               \\ \hline
\rowcolor[HTML]{EFEFEF} 
DaCy               & Medium          & 0.626                        & 0.643                        & 0.609                        \\ \hline
\rowcolor[HTML]{FFFFFF} 
DaCy               & Small           & 0.514                        & 0.48                         & 0.555                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
spaCy              & Large           & 0.485                        & 0.445                        & 0.533                        \\ \hline
\rowcolor[HTML]{FFFFFF} 
spaCy              & Medium          & 0.492                        & 0.468                        & 0.519                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
spaCy              & Small           & {\color[HTML]{000000} 0.319} & {\color[HTML]{000000} 0.321} & {\color[HTML]{000000} 0.318} \\ \hline
\end{tabular}


==> tabs/sota_tags.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{cc|c|c|c|}
\cline{3-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                                          & \cellcolor[HTML]{FFFFFF} & LOCATION       & ORGANIZATION   & PERSON         \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Large                    & 0.883          & 0.863          & 0.871          \\ \cline{2-5} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Medium                   & 0.832          & 0.851          & 0.872          \\ \cline{2-5} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}DaCy fine-grained}} & Small                    & 0.793          & 0.781          & 0.833          \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}NbAI-Lab}                            & Base-ner-scandi          & \textit{0.793} & 0.457          & 0.699          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Large                    & \textbf{0.835} & \textbf{0.501} & \textbf{0.735} \\ \cline{2-5} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Medium                   & 0.739          & \textit{0.477} & \textit{0.703} \\ \cline{2-5} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}DaCy}}              & Small                    & 0.667          & 0.378          & 0.515          \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Large                    & 0.629          & 0.281          & 0.607          \\ \cline{2-5} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                    & Medium                   & 0.649          & 0.31           & 0.579          \\ \cline{2-5} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}spaCy}}             & Small                    & 0.435          & 0.225          & 0.31           \\ \hline
\end{tabular}


==> tabs/sota_tags_no_fine_grained.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\centering
\begin{tabular}{lccc}
\topruel
\rowcolor[HTML]{EFEFEF} 
\textbf{Model}  & \textbf{LOC} & \textbf{ORG} & \textbf{PERSON} \\ 
\midrule
\midrule
\rowcolor[HTML]{FFFFFF} 
Base-ner-scandi & \textit{0.79}     & 0.46                  & 0.70            \\    
\rowcolor[HTML]{EFEFEF} 
DaCy large (0.1.0)     & \textbf{0.84}     & \textbf{0.50}         & \textbf{0.74}   \\    
\rowcolor[HTML]{FFFFFF} 
DaCy medium (0.1.0)    & 0.74              & \textit{0.48}         & \textit{0.70}   \\    
\rowcolor[HTML]{EFEFEF} 
DaCy small (0.1.0)     & 0.67              & 0.38                  & 0.52            \\    
\rowcolor[HTML]{FFFFFF} 
spaCy large (3.5.0)    & 0.63              & 0.28                  & 0.61            \\    
\rowcolor[HTML]{EFEFEF} 
spaCy medium (3.5.0)   & 0.65              & 0.31                  & 0.58            \\    
\rowcolor[HTML]{FFFFFF} 
spaCy small (3.5.0)    & 0.44              & 0.23                  & 0.31            \\    
\end{tabular}

